CoverNet: Multimodal Behavior Prediction using Trajectory Sets

We present CoverNet, a new method for multimodal, probabilistic trajectory prediction for urban driving. Previous work has employed a variety of methods, including multimodal regression, occupancy maps, and 1-step stochastic policies. We instead frame the trajectory prediction problem as classification over a diverse set of trajectories. The size of this set remains manageable due to the limited number of distinct actions that can be taken over a reasonable prediction horizon. We structure the trajectory set to a) ensure a desired level of coverage of the state space, and b) eliminate physically impossible trajectories. By dynamically generating trajectory sets based on the agent's current state, we can further improve our method's efficiency. We demonstrate our approach on public, real-world self-driving datasets, and show that it outperforms state-of-the-art methods.

==> sections/supplementary_cvpr_initial_submission.tex <==
% !TEX root = ../covernet.tex

\appendix
\title{Supplementary Materials}

\section{Trajectory set visualization}

Figure~\ref{fig:trajectory-set-visualization} visualizes the trajectory sets for fixed, hybrid, and dynamic trajectory set generation functions to better understand the space CoverNet learns to classify over.
We present the fixed trajectory sets for different coverage levels and the dynamic trajectory sets for a fixed coverage level but varying speeds.

\begin{figure*}
\begin{center}
\includegraphics[width=0.65\linewidth]{figures/trajectory_set_visualization.png}
\end{center}
\vspace{-3mm}
\caption{Visualization of fixed, hybrid, and dynamic trajectory sets for different coverage levels on the internal dataset for a $6$ second prediction horizon.}
\label{fig:trajectory-set-visualization}
\end{figure*}

\section{Visualization}

In Figure~\ref{fig:same-image-examples}, we add an extra visualization of a scene overlaid with predictions from our top models, compared against predictions from the implemented baselines.
The image represents the same scene rendered across all models.
We note that our prediction horizon is six seconds.
As such, the predictions do not reflect collisions as the pedestrians in the scene will have crossed the road before our vehicle reaches the pedestrian pose reflected in the images.

We emphasize that the CoverNet predictions do not include straight trajectories due to the slowing down of the vehicle before the curve.
When visualized as a video (see attached), CoverNet first predicts straight trajectories, followed by predicting left turn trajectories when the vehicle starts slowing down.
In terms of contrasting between CoverNet and the regression baselines, we highlight the smoothness of the trajectories predicted by our model.
Figure~\ref{fig:same-image-examples} also suggests that the different alternatives for left turns are better captured by CoverNet than by the baseline models.

\begin{figure*}
    \centering
    \subfloat[][CoverNet, fixed, $\varepsilon = 2$, 1937 modes]{%
        \includegraphics[width=0.3\textwidth]{figures/same_image/constant_epsilon_2.png}%
        %\label{fig:fixed-trajectory-set}%
        }%
    \subfloat[][CoverNet, hybrid, 1024 modes]{%
        \includegraphics[width=0.3\textwidth]{figures/same_image/hybrid.png}%
        \label{fig:dynamic-trajectory-set}%
        }%
    \subfloat[][CoverNet, dynamic $\varepsilon = 3$, 342 modes]{%
        \includegraphics[width=0.3\textwidth]{figures/same_image/dynamic.png}%
        \label{fig:dynamic-trajectory-set}%
        }%
    \hfill%
    \subfloat[][MTP~\cite{cui2019multimodal}, 3 modes]{%
        \includegraphics[width=0.3\textwidth]{figures/same_image/mtp_3.jpg}%
        %\label{fig:fixed-trajectory-set}%
        }%
    \subfloat[][MultiPath~\cite{cui2019multimodal}, dynamic, 16 modes]{%
        \includegraphics[width=0.3\textwidth]{figures/same_image/mp_16_dynamic.jpg}%
        \label{fig:dynamic-trajectory-set}%
        }%
    \subfloat[][MultiPath~\cite{cui2019multimodal}, 64 modes]{%
        \includegraphics[width=0.3\textwidth]{figures/same_image/mp_64_fixed.jpg}%
        \label{fig:dynamic-trajectory-set}%
        }%
    \caption{Examples of predicted trajectories on the same scene. The top row includes our CoverNet models, ranging from fixed to dynamic. The bottom row includes the baselines we compare against, as well as our dynamic templates variation. Objects in the world are rendered up to the current time.}
    \label{fig:same-image-examples}
\end{figure*}

\section{\ade{1} over the prediction horizon}

In Figure~\ref{fig:min-ade-over-horizon}, we show the \ade{1} for the best regression and CoverNet models to demonstrate how the performance of the different methods scales with time. We note that all of the methods show similar performance over time for the most likely mode.

\begin{figure}[H]
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/min_ade_over_horizon.png}
\end{center}
\vspace{-3mm}
\caption{The \ade{1} over the prediction horizon for the best regression and CoverNet models on our internal dataset.}
\label{fig:min-ade-over-horizon}
\end{figure}

